TRACE: Evaluating Execution Efficiency of LLM-Based Code Translation

While Large Language Models (LLMs) have substantially improved the functional correctness of code translation, the critical dimension of execution efficiency remains overlooked. We present \textbf{\textsc{Trace}}, the first benchmark to explicitly assess efficiency in LLM-translated code. \textsc{Trace} includes 1,000 efficiency-critical tasks across C++, Java, and Python, each augmented with stress tests that reveal efficiency disparities often overlooked by small-scale tests. Using \textsc{Trace}, we conduct an extensive evaluation of 28 representative LLMs and highlight several key insights: 1) Correctness and efficiency are often misaligned: the correctness leader Claude-Sonnet-4-Think achieves only moderate time efficiency, outperformed by smaller open-source LLMs such as Qwen2.5-Coder-14B-Instruct. 2) Inefficiency is both prevalent and patterned: 23.5\% of correct translations suffer from notable inefficiency, mainly arising from algorithm implementation discrepancy (11.9\%), language construct mismatch (66.4\%), and resource management inefficiency (21.7\%). 3) Inference-time prompt strategies bring only modest improvements, indicating that simple prompting alone is insufficient to improve translation efficiency. Together, our results establish execution efficiency as an essential dimension of code translation and position \textsc{Trace} as a principled foundation for efficiency-oriented evaluation.

==> Code/Motivation_Example.tex <==
\begin{tabularx}{\textwidth}{@{}X@{\hspace{8pt}}X@{}}
\begin{bluebox}[title=Source Code]
\begin{lstlisting}[language=C++]
int gcd ( int a, int b ) {
if ( a == 0 ) return b;
if ( b == 0 ) return a;
int k;
for ( k = 0;
( a | b ) & 1 == 0;
++ k ) {
a >>= 1; b >>= 1;
}
while ( a & 1 == 0 ) a >>= 1;
do {
while ( b & 1 == 0 ) b >>= 1;
if ( a > b ) swap ( a, b );
b = ( b - a );
} while ( b != 0 );
return a << k;
}
\end{lstlisting}
\end{bluebox}
&
\multirow{2}{*}{%
  \begin{minipage}[t]{\linewidth}
    \begin{bluebox}[title=Target Code]
\begin{lstlisting}[language=Python]
def gcd (a, b):
if a == 0: return b
if b == 0: return a
k = 0
while (a | b) & 1 == 0:
a >>= 1
b >>= 1
k += 1
while a & 1 ==0:
a >>= 1
while b & 1 == 0
<<<<<<<<CodeLlama-34B-Instruct-hf
:
b >>= 1
while b != 0:
if a > b:
a, b = b, a
b = b - a
==========
while b != 0:
while b & 1 == 0:
b >>= 1
if a > b:
a, b = b, a
b = b - a
>>>>>>>>GPT-4o-mini
return a << k
\end{lstlisting}
    \end{bluebox}
  \end{minipage}
}
\\[8pt]

\begin{pinkbox}[title=Execution Profile]
\begin{lstlisting}
Small Tests 0.018s v.s 0.018s
a=37, b=93
...
int gcd ( int a, int b ) {
if ( a == 0 ) return b;
if ( b == 0 ) return a;
int k;
for ( k = 0;
( a | b ) & 1 == 0;
++ k ) {
a >>= 1; b >>= 1;
}
while ( a & 1 == 0 ) a >>= 1;
do {
while ( b & 1 == 0 ) b >>= 1;
if ( a > b ) swap ( a, b );
b = ( b - a );
} while ( b != 0 );
return a << k;
}
def gcd (a, b):
if a == 0: return b
if b == 0: return a
k = 0
while (a | b) & 1 == 0:
a >>= 1
b >>= 1
k += 1
while a & 1 ==0:
a >>= 1
while b & 1 == 0
<<<<<<<<CodeLlama-34B-Instruct-hf
:
b >>= 1
while b != 0:
if a > b:
a, b = b, a
b = b - a
==========
while b != 0:
while b & 1 == 0:
b >>= 1
if a > b:
a, b = b, a
b = b - a
>>>>>>>>GPT-4o-mini
return a << k
Source Code In C++ Python Translation
Stress Tests 11.200s v.s 0.018s
a=2147483647, b=214748362
\end{lstlisting}


==> Figure/aaa.tex <==
% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.98\textwidth]{Figure/Method_Overview.pdf} 
% \caption{An overview of \textsc{Tracy}'s LLM-driven two-stage construction pipeline.}
% \label{figure:methodology_overview}
% \end{figure*}

==> Table/Taxonomy.tex <==
% --- 表格代码 ---
\begin{table*}[t!]
\centering
\caption{A Taxonomy of Inefficiencies in LLM-based Code Translation.}
\label{table:taxonomy}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\linewidth}{@{} >{\raggedright\arraybackslash}X @{}}
\toprule
% --- Major Category 1 ---
\textbf{\best{1. Algorithm Implementation Discrepancy}} \\ \addlinespace[4pt]
\quad \textbf{1.1 Asymptotic Complexity Degradation} \\
\quad \textit{Description:} The translated code preserves correctness but adopts an algorithm with worse asymptotic complexity than the source. \\
\quad \textit{Example:} Translating a linear in-place algorithm into one that repeatedly concatenates immutable strings, degrading complexity from $O(N)$ to $O(N^2)$. \\
\cdashline{1-1}
\quad \textbf{1.2 Omission of Target-Language Idioms} \\
\quad \textit{Description:} The translation ignores efficient idioms or optimized library routines available in the target language. \\
\quad \textit{Example:} Re-implementing a manual search instead of using the built-in \texttt{std::max\_element} in C++. \\

\midrule

% --- Major Category 2 ---
\textbf{\best{2. Language Construct Mismatch}} \\ \addlinespace[4pt]
\quad \textbf{2.1 Suboptimal Data Structure Selection} \\
\quad \textit{Description:} The chosen data structure is functionally correct but asymptotically or practically inferior for the required operations. \\
\quad \textit{Example:} Mapping Java’s \texttt{HashMap} (amortized $O(1)$) to C++’s \texttt{std::map} ($O(\log N)$) instead of \texttt{std::unordered\_map}. \\

\cdashline{1-1}
\quad \textbf{2.2 Inefficient API/Pattern Usage} \\
\quad \textit{Description:} The translation relies on heavyweight APIs or programming patterns that introduce unnecessary overhead. \\
\quad \textit{Example:} Translating C++ \texttt{vector<vector<int>>(n, vector<int>(n,1))} into Python \texttt{[[1 for \_ in range(n)] for \_ in range(n)]}, which is slower than the idiomatic \texttt{[[1]*n for \_ in range(n)]}. \\

\midrule

% --- Major Category 3 ---
\textbf{\best{3. Resource Management Inefficiency}} \\ \addlinespace[4pt]
\quad \textbf{3.1 Inefficient Data Representation} \\
\quad \textit{Description:} Primitive or compact source representations are replaced with memory-intensive object-based equivalents in the target language. \\
\quad \textit{Example:} Translating C++ \texttt{long} into Java \texttt{BigInteger}, which incurs excessive object allocations and memory overhead. \\
\cdashline{1-1}
\quad \textbf{3.2 Non-Idiomatic Memory Management} \\
\quad \textit{Description:} The translation adopts manual or unsafe memory practices instead of modern, idiomatic abstractions in the target language. \\
\quad \textit{Example:} Using raw \texttt{new}/\texttt{delete} in C++ instead of RAII containers or smart pointers. \\
\bottomrule
\end{tabularx}
\end{table*}
